Generating Holistic 3D Human Motion from Speech

This work addresses the problem of generating 3D holistic body motions from human speech. Given a speech recording, we synthesize sequences of 3D body poses, hand gestures, and facial expressions that are realistic and diverse. To achieve this, we first build a high-quality dataset of 3D holistic body meshes with synchronous speech. We then define a novel speech-to-motion generation framework in which the face, body, and hands are modeled separately. The separated modeling stems from the fact that face articulation strongly correlates with human speech, while body poses and hand gestures are less correlated. Specifically, we employ an autoencoder for face motions, and a compositional vector-quantized variational autoencoder (VQ-VAE) for the body and hand motions. The compositional VQ-VAE is key to generating diverse results. Additionally, we propose a cross-conditional autoregressive model that generates body poses and hand gestures, leading to coherent and realistic motions. Extensive experiments and user studies demonstrate that our proposed approach achieves state-of-the-art performance both qualitatively and quantitatively. Our novel dataset and code will be released for research purposes at https://talkshow.is.tue.mpg.de.

==> paper/FIG_01_architecture_motion_generation.tex <==
\newcommand{\architectureCaption}{
(draft) The architecture of our audio-driven 3D human motion generation model.
}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth*4/9]{figs/speech-driven-generater.pdf}
    
    
    \caption{\architectureCaption}
    \label{fig:architecture}
\end{figure}



==> paper/FIG_09_perceptual_study_prototype.tex <==
\newcommand{\perceptualPrototypeCaption}{
\lhl{Perceptual Study UI. Is the reconstructed results real or not?}
}


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figs/perceptual_question.png}
    \caption{\perceptualPrototypeCaption}
    \label{fig:perceptual_prototype}
\end{figure}



==> paper/FIG_ours_vs_ik.tex <==
\begin{figure}[t]
    \centering
    % \includegraphics[width=\textwidth,height=10cm]{example-image-a}
    \includegraphics[width=\columnwidth]{figs/Talkshow_rebuttal.pdf}
    \vspace{-19pt}
    % \caption{Composed from two image with a 3-frame interval. The columns from left to right are: original video, our reconstruction result, visualization from [19], and SMPLX result obtained from inverse kinematics of [19]. It can be seen that [19] and its inverse kinematics results contain some obvious detection errors (such as the left hand of [19]), show significant jitter when observed over time dimension, and exhibit changes in body shape information such as bone length. In contrast, our results consider shape consistency and thus are more reasonable and smooth visually and qualitatively.}
    % \footnotesize
    \caption{\footnotesize{a) Holistic body reconstruction compared to Habibie et.al.; b) Our generated holistic body motion from the song ``Jingle Bells''.}}
    \vspace{-20pt}
    \label{fig:rebuttal}
\end{figure}


==> paper/SEC_06_discussion.tex <==
\section{Discussion}

% \paragraph{limitation.}

% reconstruction. \lhl{Our method is robust most of the time. But face tracking would fail when there are extreme occlusion, e.g. where the hand covers large area of the face. When two hand are too close to each other or there is fast hand motion with image blur, 2d hand pose estimation may not robust, resulting the quality of hand pose reconstruction is low. Our method can only handle static camera cases currently.}

% audio2motion. \YF{Our face generator can generate appropriate expression according to the audio, however, there are still a few artificial results observed in experiment. This is mainly because facial expression is a much more complex problem than the assumption; emotion and blink should be concerned, for example. Noise samples in dataset could be another reason for the artificial results. Besides, even though our generated motions are diverse and realistic, the exact correspondence between words and hand gestures should be further explored.}


==> paper/SEC_11_rebuttal.tex <==
\noindent We thank the reviewers \Rone~(\RoneH), \Rtwo~(\RtwoH), and \Rthree~(\RthreeH) for their constructive feedback.
The reviewers find that the ``high quality speech-driven body meshes \textbf{dataset}'' \textbf{[\Rone]} is ``valuable'' \textbf{[\Rtwo]} and could ``facilitate the community for further research'' \textbf{[\Rthree]}, the \textbf{pseudo labeling pipeline SHOW} could ``extend to broader fields to accommodate other relative tasks'' \textbf{[\Rone]}, and the \textbf{motion generation method} is ``well-motivated'' \textbf{[\Rone]} and ``effective'' \textbf{[\Rtwo]}. 
{\noindent}	\rule[0pt]{8.3cm}{0.1em}

% \noindent\textbf{Better Visualization [\Rone]:}
% We agree with \textbf{[\Rone]} that "the presentation could be more clear with better visualizations." Besides, we did draw the red arrows wrong in Figure 3. We will fix the figure and present better visualization in the revised version.

% \noindent\textbf{More Clear Figures [\Rone]:}
\noindent\textbf{Figures [\Rone]:}
% We thank \textbf{[\Rone]} for pointing out a typo in Fig. 3 and providing suggestions to improve Fig. 4. They will be addressed in the revised version.
We will fix the typo and improve Fig. 4.

\noindent\textbf{Video Occlusion [\Rone]:}
% \lhl{For the talk show scenario, where the lower body is mostly obscured and the subject is primarily sitting or standing, we replaced the lower body pose with a fixed pose after labeling.} 
% We tried to generate motions with a song as input. The generated facial expressions are well-aligned with the song, and the generated body motions are conversational gestures aligned with the audio dynamics, which is reasonable.
% The SHOW algorithm can be applied to any type of video, not just talk shows, and the TalkSHOW algorithm trained on this dataset can also be applied to any type of audio.}
% \yd{Majority of the occlusions are located at lower body, for which we use a fixed pose (sitting?standing?).}
We use a fixed pose (sitting or standing) for the invisible lower body; we will clarify in Sup.~Mat.
% In this work we do not explicitly model the lower body pose, since they are hardly correlated with the input speech.
% \yd{One of the reasons to collect dataset from talk show videos is because talk show covers a wide range of topics, gesturing styles, background noises, etc. 
% Trained by this dataset, our model can generalize to other types of audios, even songs. For example, the generated motions from a song (never shown in the training set) are very reasonable: the generated facial expressions are well-aligned with the phonemes, and the generated body poses are aligned with the rhythm and dynamics. More video demonstrations will be added to the supplementary materials.}

\noindent\textbf{Generalization to Other Types of Audio [\Rone]:}
% Collecting datasets from talk show videos can help train a model to generalize to other audio types, because talk show covers a wide range of topics, gesturing styles, background noises, etc. 
% The trained model can generate reasonable motions, such as facial expressions aligned with phonemes and body poses aligned with rhythm and dynamics, even for \textbf{songs} not seen in the training set. 
% \TODO{Add one example: illustration.} 
\Fref{fig:rebuttal} b) shows samples of the generated motion for the song ``Jingle Bells''. 
% The generated motions with the song ``Jungle Bells'' are shown in \Fref{fig:rebuttal}. 
% TalkSHOW can generate reasonable motions, such as facial expressions aligned with phonemes and body poses aligned with rhythm and dynamics.
TalkSHOW generates plausible body motions aligned with the rhythm, and  facial expressions aligned with phonemes.
We will add the example to the video.

% \noindent\textbf{Ablation Study [\Rone, \Rthree]:}
% \noindent\textbf{{Comparison between VQ-VAE and VQ-VAEs [\Rone]:}}
\noindent\textbf{{VQ-VAE vs.~VQ-VAEs [\Rone]:}}
% In Fig. 6, the size of VQ-VAEs with $|Z|=1024$ is much lower than that of a VQ-VAE with $|Z|=16384$, while the former achieves lower reconstruction error.
% In our experiments, the reconstruction error of a single VQ-VAE with codebook size $|Z|=170000$ is still much higher than VQ-VAEs with $|Z|=1024$ (5.74 v.s. 5.01), and the former requires more than 11GB of GPU memory but the latter only requires around 4GB on a 1080Ti GPU card.
% Requested by \Rone, we train a single VQ-VAE model with a quite large codebook size $|Z|=170,000$. 
As suggested, we train a single VQ-VAE model with a large codebook size $|Z|=170,000$. 
%The reconstruction error is still higher than that of our VQ-VAEs with small codebook size $|Z|=1,024$ (5.74 v.s. 5.01), and it consumes more GPU memory (11GB vs 4GB) on a 1080Ti GPU card.
%
% 
% Similar as 1
Compared to our VQ-VAEs with small codebook sizes $|Z|=1,024$, the VQ-VAE model has a higher reconstruction error (5.74 vs.~5.01), and it costs more GPU memory (11GB vs.~4GB) on a 1080Ti GPU, similar to Fig.~6.
%

% In Fig. 6, The reconstruction error of a single VQ-VAE model with a quite large codebook size $|Z|=16384$ is still higher with our VQ-VAEs with small codebook size $|Z|=1,024$ \TODO{5.74 v.s. 5.01}, and it consumes more GPU memory (11GB vs 4GB) on a 1080Ti GPU card.
% In our experiments, the reconstruction error of a single VQ-VAE with codebook size $|Z|=170000$ is still much higher than our VQ-VAEs with small codebook size $|Z|=1024$ (5.74 v.s. 5.01) , and the former requires more than 11GB of GPU memory but the latter only requires around 4GB on a 1080Ti GPU card.
% \TODO{Add one answer.}
% We provide the ablation study for the number and size of codebooks in L.780-804 and Fig.6.
% \noindent Ablation studies proposed by \textbf{[\Rthree]} had been presented in the paper. The performance of VQ-VAE with a single codebook was demonstrated in Figure 6. The effect of cross-condition was demonstrated in L.793-804.
% Our proposed VQ-VAEs of two codebooks with cross-condition achieve lower reconstruction errors and higher realistic scores.
% --------------------------------------------
% \noindent\textbf{Separated Modeling and Feature Selection for Face and Body [\Rtwo]:}
\noindent\textbf{Separate Face and Body Animation [\Rtwo]:}
% The independent modeling approach was chosen because it assumes facial expressions, especially the mouth region, should strongly correlate with speech audio, while body motions are less correlated or even uncorrelated. (L.149-154). 
% 
As the face and body are animated by the same audio signal, we did not see any out-of-sync issues between body, hands, and face.
% Due to the alignment of facial expressions with audio features and the body motion with the audio rhythm, we did not see any out-of-sync issues between faces and 
% We did not see clear out-of-sync issues, \TODO{because the facial expression is well aligned with the phonemes of the audio, while the body motion with the rhythm of the audio.}
 % in our massive generated motions from our independent modeling approach.
% However, there are relations between face and body motions indeed, such as emotion. Therefore, we agree with \textbf{[\Rtwo]} that such a modeling might cause out-of-sync to some degree, and the correlation between face and body motions should be further explored in future work.
% However, there are connections between facial and body motions, such as emotions. 
% Further exploration of the correlation between facial and body motions is one of our future work.
Modeling emotions, which likely have correlated facial and body motion, is an interesting direction for future work, which we will discuss.
% \TODO{And FaceFormer and MeshTalk both work for face only. [not generative models.]}
% \noindent We use the Wav2Vec feature to provide a fine-grained feature for face-audio alignment and use the MFCC feature to provide a rhythm and dynamics feature for body motion. In our experiments, the convergence speed is quite slow when only using the Wav2Vec feature to generate body motion
% 
% \noindent\textbf{Feature Selection for Face and Body [\Rtwo]:}
% Faceformer and MeshTalk with different features, both work for face motion generation.
% Combination problem.
% The independent modeling approach was chosen because it assumes facial expressions, especially the mouth region, should strongly correlate with speech audio, while body motions are less correlated or even uncorrelated. (L.149-154). 
% Wav2Vec features are used for precise face-audio alignment, while MFCC features provide rhythm and dynamics information for body motion, see L.478-481.
% Our designed facial motion generator and body motion generator are not the combination of FaceFormer and MeshTalk, because the architectures of them are totally different.
% \TODO{We design our facial motion generator as a simple deterministic auto-encoder and body motion generator as a compositional VQ-VAEs generative model, which is totally different from a combination of the transformed based FaceFormer and a single VQ-VAE based MeshTalk.}
Our facial motion generator is a deterministic encoder-decoder model; the body motion generator is a compositional VQ-VAEs model. 
This differs from a combination of the transformer-based FaceFormer and the single VQ-VAE-based MeshTalk.
Intuitively, Wav2Vec features are used for face-audio alignment, while MFCC features provide rhythm and dynamics information for body motion (L.478-481).
Using Wav2Vec for body motion generation results in slow convergence.
We will clarify.

% \noindent\textbf{User Study [\Rtwo]:}
% \TODO{add description.}
% \lhl{For the user study setup of the reconstruction result, we randomly selected 10 videos from each of 4 speakers for a total of 40 videos and arranged them side by side with their corresponding original videos. In the questionnaire, we emphasized for the participants to answer based on the main focus of the specific part, such as body shape, facial expression, body and hand movements, and whether they match the original video. For the generation result, we randomly selected 10 audio segments from each speaker in the test set to generate a total of 40 videos for TalkSHOW and [19], respectively. These videos were randomly spliced together into one video and all potentially biased text information was removed. These videos were placed in the questionnaire and participants were asked to focus on specific parts of the generation results and answer questions. Participants were randomly selected, with each individual required to respond to every question in each questionnaire, under the principle of fairness and objectivity.}

% --------------------------------------------
\noindent\textbf{Related Work [\Rthree]:}
% The paper has discussed most relevant works in Sec. 2, and we agree to discuss more, especially audio2face and other related fields that use VQ-VAE.
We will extend the related work, especially by audio2face and related VQ-VAE-based methods.


\noindent\textbf{Holistic Body Representation [\Rthree]:}
% reconstruction results;
% 
% SMPL-X represents a holistic body including body, hand and face in a unified parametric model. 
SMPL-X holistically models body, hands, and face with a unified parametric representation. 
% Compared with other formats, 2D skeletons (Ginosar et al.) and 3D skeletons (Yoon et al.), it disentangles body shape and body poses separately, which also enables broad applications.  
Compared to other formats like 2D skeletons (Ginosar et al.) or 3D skeletons (Yoon et al.), it disentangles body shape and pose, important for retargeting and animation applications.  
% 
% For instance, with SHOW's estimated SMPL-X pose parameter one can animate arbitrary body shapes, while 2D/3D keypoint representations are restricted to a single body, determined by the bone lengths. 
%The reconstructed SMPL-X body params, i.e. rotation axis-angle from SHOW, can be directly applied to arbitrary body shapes, while the 2D/3D keypoints are strictly limited by the body shape, i.e., bone length.
% And SMPL-X includes expressive face and hand compared with SMPL (Li et al.), which are also significant for communication as described in L.101-105.
Additionally, recovering 3D bodies, e.g., for VR/AR applications, from 2D/3D skeletons with inverse kinematics is not trivial. 
Compared to the SMPL-based method of Li et al., using SMPL-X enables us to consider hand articulation and facial expressions, which are essential for communication (L.101-105).
% Compared with 
% Moreover, getting a 3D mesh from 3D skeletons with inverse kinematics is not trivial. 
% In \Fref{fig:rebuttal} a), the hand poses and head poses from Habibie et.al reconstructed with 3D skeletons or body mesh are less accurate with larger jitter than ours.
% Compared results on a video will be added into the Sup.Mat.
% In contrast, SHOW leverages several simple but effective practices in Sec.3.2. to achieve more stable and accurate holistic body meshes.
We will clarify. 

\noindent\textbf{Difference from Existing Methods [\Rthree]:}
% 
% \TODO{Learning difficulty. [Estimated 3D skeletons.]}
% Directly generated SMPL-X body params, i.e. rotation axis-angle from TalkSHOW, can be directly applied to arbitrary body shapes, while the 2D/3D keypoints is strictly limited by the body shape, i.e., the length of each bone. 
% employs several simple but effective improvements, i.e., extending the data term and regularization of SMPLify-X (L.314-384) and achieves nice reconstruction results, as demonstrated in Table 3.}
% Besides, SMPL-X params could be transformed into more realistic 3D human meshes than keypoints, as shown in Figure 1.
% Moreover, more conditions such as mesh collision could be explored in conversation gesture task since human mesh is easy to get through SMPL-X model.
% SMPL-X data of Li et al. is re-targeted from keypoints and therefore less accurate. Besides, their SMPL-X data does not include face and hand data. 
% \lhl{In contrast, our data is \textit{holistic} and obtaining high-quality, holistic reconstruction data including faces and hands is a challenging task. To achieve this, we have put in considerable effort. Our reconstruct pipeline employs simple but effective improvements and achieves better reconstruction results than previous SOTA in practice.}
% \noindent\textbf{b) Difference with Habibie et al.:}
\noindent\textbf{a) Habibie et al.:}
% Comparing to Habibie et al. in which each part is collected separately in L.241-244, we reconstructed whole-body 3D meshes in a connected way to improve the whole-body consistency. 
% Habibie et al. represent body, hand, and face separately (L.241-244), which lacks connection between head and face, wrist and fingers, compared with ours see \fref{fig:rebuttal} a).
Habibie et al.~represent body, hands, and face separately (L.241-244).
The lack of connection between body and face/hands results in unnatural poses of the face/hands w.r.t.~the body. 
\Fref{fig:rebuttal} a) shows that the hand and head poses of the body mesh, reconstructed from their estimated 3D skeleton, are less accurate than ours. 
Generated video results are further jittery.
In contrast, SHOW generates more stable and accurate holistic body meshes.
We will add more comparison sequences to the video. 
% , the hand poses and head poses from Habibie et.al reconstructed with 3D skeletons or body mesh are less accurate with larger jitter than ours.
%, which lacks connections between neck and head, and wrist and fingers, compared with ours see \fref{fig:rebuttal} a).
% Moreover, we designed a hierarchical framework considering different nature of different body parts , which leads to more realistic and reasonable whole-body motions.
%
% And our intuition and derived network design are different from Habibie et al. in L149-161. 
Beside the body representation and the result quality, our network design and intuition behind our framework differ from Habibie et al. (L149-161).
% Also see the answer of "Architecture Design & Feature Selection".
We model the face deterministically, while the body and hands are modeled in a generative way. 
Given one speech sequence, our method generates multiple diverse realistic body and hand motions accompanied by one facial expression.
However, Habibie et al. models body, hand, and face jointly in a deterministic encoder-decoder, which can only generate one body, hand and face motion.
We will clarify this. % in related work and introduction.
% 
% \noindent\textbf{c) Differences with VQ-VAE based Works: }
\noindent\textbf{b) VQ-VAE-Based Works [\Rthree]: }
Bailando outputs the same result given the same audio input, while our method generates diverse results by sampling from a probability distribution. 
To ensure body and hand synchronization, we design a more sophisticated cross-condition module that considers the current state (L582-585).
% On this basis, to keep the body and hand synchronized, we designed a more delicate cross-condition module which takes into account the current state . 
% Regarding VQ-Text2Sign, it adopted a code-shared VQ-VAE rather than multiple VQ-VAEs.
In comparison, the VQ-Text2Sign uses a shared code VQ-VAE instead of multiple VQ-VAEs.
% 1) Architecture: this paper extends the one shot generation framework of Habibie et al. with a well-motivated, hierarchical framework to account for different nature of different body parts as pointed out by \textbf{[\Rone]}.
% 2) Data: the difference of data has been demonstrated above. 

\input{paper/FIG_ours_vs_ik}

\input{tables/TAB_10.tex}

\noindent\textbf{More Metrics \& More Comparison [\Rthree]:}
% \TODO{add conclusion.}
% \TODO{More comparison is shown in Table \ref{tab:new_metric}. FGD is adopted to measure the motion realism instead of FTD. The effectiveness of Beat Consistency is limited because the change of motion could not be fully represented by the change of angle between bones. Variance is adopted to measure the diversity as described in L.645-647. As illustrated in Table \ref{tab:new_metric}, our method with cross-condition achieves considerable results in both realism and diversity.}
As suggested by \Rthree, we add FGD to measure the motion realism (more commonly used than FTD) and beat consistency to measure the alignment between the generated body motion and input audio, and compare with another audio-to-body motion baseline [28] in \tref{tab:new_metric}.
Our method outperforms the baselines in all these metrics and generates more diverse body motions, better aligned with the input audio.
We will add this.
% We had adopted commonly used metrics in speech-driven motion generation [2, 30, 44, 49]. Results with the metrics mentioned by \textbf{[\Rthree]} are shown in Table \ref{tab:new_metric}.
% Due to time reasons, we only compared our method with the most relevant work and several baselines. We will consider to add more comparison in the revised version.

% {\noindent}	\rule[0pt]{8.3cm}{0.1em}
\noindent\textbf{Ablation Studies for w/o VQ-VAEs and Cross-Condition Modeling [\Rthree]:} 
Comparisons are in L780-804 and Fig. 6.


% \vspace{-0.6 em}
% \noindent\rule{\columnwidth}{1pt}
% \noindent
% We will integrate all feedback into the final version. 
% \textbf{We renew our promise to release TalkSHOW’s code and data to foster future research on speech to holistic body motion.}




\clearpage






% \noindent\textbf{Novelty [\Rthree]:}
% In this section, we will demonstrate the novelty of this work, which is concerned by \textbf{[\Rthree]}. 
% Firstly, we provide a medium-size dataset and a pseudo labeling pipeline named SHOW, in which the latter might be overlooked by \textbf{[\Rthree]}. With SHOW, we can simply extend our dataset to multi-subjects and multi-scenarios. Besides, as pointed out by \textbf{[\Rone]}, SHOW could be "extend to broader fields to accommodate other relative tasks", e.g., dyadic conversation. Experimental results confirm that such a pipeline is feasible and practical.
% Regarding \textbf{[\Rthree]}'s concern of data format, our SMPL-X-based data could be directly transformed into a realistic 3D human mesh, while the 2D/3D skeleton-based data could not, and as proposed by \textbf{[\Rthree]}, "the learning difficulty has no evident difference."
% Secondly, we present a method to drive holistic 3D human motion with audio, in which the body\&hand motion and facial expression are modeled separately considering the nature of each part, which is quite different from the previous method [19]. We agree with \textbf{[\Rthree]} that VQ-VAE or vector quantized idea has been used in motion generation task. Nevertheless, there are many differences between our method and existing methods, e.g., input/output modality and modeling method. This work confirms the effectiveness of using separate VQ-VAEs to generate body\&hand motions from speech audio, which has never been explored before.


% \noindent \lhl{Regarding \textbf{[\Rthree]}'s mention of "extending the speech audio-driven gesture dataset is also explored recently, e.g., BEAT," it is clear that our algorithm and dataset are superior. SHOW is able to generalize to a wide range of internet videos, resulting in high-quality and easily scalable pGT datasets. In contrast, the BEAT dataset utilizes MoCap, which is costly, limited in quantity, and in-house, and thus inferior to our in-the-wild dataset.}

% Bailando, a music-to-dance method, use two codebooks to encode upper and lower body separately. However, Bailando outputs deterministic result when take as input the same audio, while our method samples on the possibility distribution to generate diverse results. On this basis, to keep the body and hand synchronized, our cross-conditioning module takes into account the current state, i.e., the current hand state is influenced by the current body state (L.582-583). 

% Additionally, a user study was conducted to evaluate the quality of our reconstruction and generation methods. We agree with \textbf{[\Rthree]} that there are other metrics in motion generation. Regarding \textbf{[\Rthree]}'s concern of limited compared works, the comparison between our method and the most relevant work [19] has been conducted, and other works are less relevant.

==> tables/TAB_02.tex <==
% \begin{table}
%     \centering
%     %\small
%     \footnotesize
    
%     \begin{tabular}{l|cc|ccc}
%     \toprule
%     \multirow{3}{*}{Method}   & \multicolumn{2}{c|}{Face} & \multicolumn{3}{c}{Motion} \\
%     & \tabincell{c}{Jaw \\ Dist. $\downarrow$} 
%     & \tabincell{c}{E.L. \\ Dist. $\downarrow$}  
%     & \tabincell{c}{Realistic \\ Score $\uparrow$} 
%     & \tabincell{c}{Syncing \\ SLVD $\downarrow$} 
%     & \tabincell{c}{Diversity \\ Dist. $\uparrow$}\\ \hline
%     MFCC-Based                  & 0.0009    & 0.1679    &0.4137     &  0.3445   & 9.4585\\ \hline
%     \textbf{Wav2Vec-Based}      & 0.0007    & 0.1358    &0.4842     & 0.3383   & 9.4379\\ \hline
%     \end{tabular}

%     \caption{The performance of MFCC and Wav2Vec feature on face and motion generation respectively.} 
%     \label{expression}
% \end{table}
\begin{table}
    \centering
    %\small
    \footnotesize
\begin{tabular}{l|cc}
    \toprule
    \tabincell{l}{Method}       
    & \tabincell{c}{Jaw L1 $\downarrow$} 
    & \tabincell{c}{E.L. L1 $\downarrow$}  \\ \hline
    MFCC-Based                  & 0.0009                & 0.1679 \\ \hline
    \textbf{Wav2Vec-Based}      & 0.0007                & 0.1358 \\ \hline
\end{tabular}
   \caption{(abolished)The performance of face generator using MFCC and Wav2Vec features.} 
    \label{expression}
\end{table}

==> tables/TAB_03.tex <==
\begin{table}
    \centering
    %\small
    \footnotesize
    
    \begin{tabular}{l|ccc}
    \toprule
    \tabincell{l}{Method} 
    & \tabincell{c}{Realistic \\ Score $\uparrow$} 
    & \tabincell{c}{Syncing \\ SLVD $\downarrow$} 
    & \tabincell{c}{Diversity \\ Dist. $\uparrow$} \\ \hline
    Audio Encoder-Decoder                       & 0.2141 & 0.3321  & 0  \\ \hline
    Audio VAE                                   & 0.1820 & 0.2696  & 1.7420 \\ \hline
    Audio+Motion VAE                            & 0.2397 & 0.2875  & 3.7560 \\ \hline
    % VQ-VAE                                      & 0.4484 & 0.2254  & 9.4275 \\ \hline
    VQ-VAE w/o BHC modeling                    & 0.4093 & 0.4628 & 11.0852 \\ \hline
    \textbf{VQ-VAE w/ BHC modeling}           & 0.4137 & 0.3445  & 9.4585 \\ \hline
    \end{tabular}

    \caption{Quantitative results for the speech to motion translation task.} 
    \label{motion}
\end{table}

==> tables/TAB_04.tex <==
\begin{table}
    \centering
    %\small
    \footnotesize
    
    \begin{tabular}{l|ccccc}
    \toprule
    \tabincell{l}{Method} 
    & \tabincell{c}{Jaw \\ Dist. $\downarrow$} 
    & \tabincell{c}{E.L. \\ Dist. $\downarrow$} 
    & \tabincell{c}{Realistic \\ Score $\uparrow$} 
    & \tabincell{c}{Syncing \\ SLVD $\downarrow$} 
    & \tabincell{c}{Diversity \\ Dist. $\uparrow$} \\ \hline
    SG3D                  & 0.0008                & 0.1428              & 0.1466                   &  0.3979                & 0                        \\ \hline
    \textbf{Our Method}   & 0.0007                & 0.1358              & 0.4137                   &  0.3445                & 9.4585                   \\ \hline
    \end{tabular}

    \caption{The comparison between SG3D \cite{habibie2021learning} and our method.} 
    \label{tab:comparison}
\end{table}

==> tables/TAB_05.tex <==
\begin{table}
    \centering
    %\small
    \footnotesize
    
    \begin{tabular}{l|cc}
    \toprule
    \tabincell{l}{Method} 
    & \tabincell{c}{Capacity \\ Dist. $\downarrow$} \\ \hline
    VQ-VAE, $|Z|=1024$   & 6.2518 \\ \hline
    VQ-VAE, $|Z|=2048$   & 5.6415 \\ \hline
    VQ-VAE, $|Z|=4096$   & 5.6232 \\ \hline
    VQ-VAE, $|Z|=8192$   & 6.17896032333374 \\ \hline
    VQ-VAE, $|Z|=16384$   & 5.701906681060791 \\ \hline
    % VQ-VAE, $|Z|=170000$ & 5.7478 \\ \hline
    VQ-VAEs, $|Z_H|=|Z_B|=1024$   & 5.0106 \\ \hline
    VQ-VAEs, $|Z_H|=|Z_B|=2048$   & 4.8137 \\ \hline
    VQ-VAEs, $|Z_H|=|Z_B|=4096$   & 4.8556 \\ \hline
    VQ-VAEs, $|Z_H|=|Z_B|=8192$   & 4.859879493713379 \\ \hline
    VQ-VAEs, $|Z_H|=|Z_B|=16384$   & 4.835285663604736 \\ \hline
    \end{tabular}

    \caption{The comparison between VQ-VAE and VQ-VAEs with different codebook size $|Z|$ and our compositional VQ-VAEs.} 
    \label{tab:compositional}
\end{table}

==> tables/sym.tex <==
\begin{table}
    \centering
    %\small
    \footnotesize
    
    \begin{tabular}{l|c}
    \toprule
    \tabincell{l}{symbol}       & \tabincell{c}{meaning} \\ \hline
    
    \\\hline

    \end{tabular}

    \caption{symbol table for paper writing.} 
    \label{tab:symbol}
\end{table}
